Towards a Semantic Characterisation of Global Type Well-formedness

We address the question of characterising the well-formedness properties of multiparty session types semantically, i.e., as properties of the semantic model used to interpret types. Choosing Prime Event Structures (PESs) as our semantic model, we present semantic counterparts for the two properties that underpin global type well-formedness, namely projectability and boundedness, in this model. As a first step towards a characterisation of the class of PESs corresponding to well-formed global types, we identify some simple structural properties satisfied by such PESs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{11}
\providecommand{\publicationstatus}{D. Costa, R. Hu (Eds.): Programming Language Approaches to\\ Concurrency and Communication-cEntric Software 2024 (PLACES'24)\\
EPTCS 401, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.401.2}{10.4204/EPTCS.401.2}}

